Uncertainty-o: One Model-agnostic Framework for Unveiling Uncertainty in Large Multimodal Models

Large Multimodal Models (LMMs), harnessing the complementarity among diverse modalities, are often considered more robust than pure Language Large Models (LLMs); yet do LMMs know what they do not know? There are three key open questions remaining: (1) how to evaluate the uncertainty of diverse LMMs in a unified manner, (2) how to prompt LMMs to show its uncertainty, and (3) how to quantify uncertainty for downstream tasks. In an attempt to address these challenges, we introduce Uncertainty-o: (1) a model-agnostic framework designed to reveal uncertainty in LMMs regardless of their modalities, architectures, or capabilities, (2) an empirical exploration of multimodal prompt perturbations to uncover LMM uncertainty, offering insights and findings, and (3) derive the formulation of multimodal semantic uncertainty, which enables quantifying uncertainty from multimodal responses. Experiments across 18 benchmarks spanning various modalities and 10 LMMs (both open- and closed-source) demonstrate the effectiveness of Uncertainty-o in reliably estimating LMM uncertainty, thereby enhancing downstream tasks such as hallucination detection, hallucination mitigation, and uncertainty-aware Chain-of-Thought reasoning.

==> sec/0_abstract.tex <==
\begin{abstract}
% Background
Large Multimodal Models (LMMs), characterized by diverse modalities, architectures, and capabilities, are rapidly emerging.
% Problem
% # explain in short what is LMM's uncertainty, what is all about
In this paper, we aim to address three key questions:
(1) Can we unveil the uncertainty of LMMs in a unified manner, regardless of the modalities, architectures, and capabilities involved?
(2) Complexity of multimodal prompts leads to confusion and uncertainty in LMMs, how can we model this complexity?
(3) LMM uncertainty ultimately reflects in multimodal responses, how can we mine uncertainty from these multimodal responses?
% Method
To answer these questions, we propose Uncertainty-o:
(1) Uncertainty-o is a unified framework for unveiling uncertainty in LMMs, independent of their modalities, architectures, and capabilities.
(2) We empirically explore multimodal prompt perturbation for unveiling LMM uncertainty, providing our insights and findings.
(3) We propose multimodal semantic uncertainty, enabling quantification of uncertainty from multimodal responses.
% Result
Experiments with 18 benchmarks across various modalities and 10 LMMs (open- and closed-source) validate the efficacy of Uncertainty-o in reliably estimating LMM uncertainty, thereby facilitating various downstream tasks, including hallucination detection, hallucination mitigation, and uncertainty-aware CoT.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
Large Multi-Modal Models (LMMs)~\cite{caffagni2024revolution,carolan2024review} significantly expand the boundaries of human-made intelligence. \textbf{(1) More modalities are continuously integrated.} Beyond the initial success of the `Text-in-Text-out' paradigm~\cite{achiam2023gpt}, LMMs now incorporate images~\cite{liu2023visual,rombach2022high}, videos~\cite{lin2023video,luo2023videofusion}, audio~\cite{radford2023robust,kreuk2022audiogen}, point clouds~\cite{xu2024pointllm,nichol2022point}, IMU~\cite{girdhar2023imagebind}, fMRI~\cite{han2024onellm}, and more~\cite{wu2024next}. \textbf{(2) Model architectures are rapidly evolving.} The foundational designs of Large Language Models (LLMs)~\cite{achiam2023gpt,brown2020language} and Diffusion Models (DMs)~\cite{rombach2022high,ho2020denoising} have been extensively adapted~\cite{liu2023visual} and integrated~\cite{wu2024self} to create more advanced and complex structures. \textbf{(3) Model capabilities have significantly improved.} LMMs can now comprehend intricate multimodal contexts and instructions~\cite{lyu2024unibind,han2024onellm}, while simultaneously generating diverse and high-fidelity content across various modalities~\cite{wu2024next,zhan2024anygpt}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{comparison.pdf}
    \caption{
    \textbf{Comparison between previous works and Uncertainty-o.}
    Uncertainty-o proficiently captures uncertainty in \textit{large multimodal models}, achieves accurate uncertainty estimation via \textit{multimodal prompt perturbation}, and harnesses \textit{multimodal semantic uncertainty} for mining uncertainty from multimodal responses.
    }
    \label{fig:comparison}
    \vspace{-15pt}
\end{figure}

When asked a question or given a task, humans not only provide an answer or take action, but also experience internal feelings-confidence or uncertainty, ease or difficulty~\cite{peterson2019human,collins2023human}. These feelings guide us in predicting outcomes and adjusting our plans accordingly~\cite{callaway2022rational,auletta2023predicting}. However, large models~\cite{liu2023visual,achiam2023gpt} still follow a basic `Prompt-In-Response-Out' pipeline, which remains raw and primitive compared to human cognition~\cite{amayuelas2023knowledge,pi2024mllm}. To bridge this gap and explore the psychology of LMMs~\cite{ke2024exploring,griffin2023large}, we focus on one critical property: LMM uncertainty~\cite{aichberger2024many,shorinwa2024survey}.

In this paper, we aim to answer 3 key questions: \textbf{(1) How can we unveil LMM uncertainty in a unified manner?} Tailoring specific design for different LMMs can lead to a complex and inflexible framework, limiting adaptability to revolving LMMs~\cite{caffagni2024revolution,carolan2024review}. \textbf{(2) How to model the correlation between complexity in multimodal prompts and LMM uncertainty?} Notably, LMM uncertainty can be significantly lifted by newly introduced modalities and the interaction between different modalities~\cite{lu2023theory,fu2022complexity}. \textbf{(3) How to mine uncertainty from multimodal responses where LMM manifests its uncertainty?} The cues are hidden in these multimodal responses~\cite{rombach2022high,kreuk2022audiogen,nichol2022point,wu2024next}, \eg, generated images~\cite{rombach2022high} or point clouds~\cite{lee2024rgb2point}, requiring effective methods to extract and quantify uncertainty.



In response to those substantial questions, we propose Uncertainty-o: \textbf{(1) Uncertainty-o, in a unified manner, unveils uncertainty in LMMs, regardless of the modalities involved, inherent architecture, and capability focus.} Notably, Uncertainty-o is also scalable and can incorporate emerged modalities, architectures, and capabilities. \textbf{(2) We empirically explore multimodal prompt perturbation for eliciting LMM uncertainty.} By causing variance at the prompt end, we can observe fluctuations in LMM responses, thereby capturing its uncertainty. We provide a comprehensive empirical analysis of perturbation for 5 commonly used modalities, including text, image, video, audio, and point cloud. Finally, we offer our findings and insights, which are modality-agnostic and can serve as a cookbook when designing perturbation for other potential modalities. \textbf{(3) We propose multimodal semantic uncertainty, which can mine uncertainty from multimodal responses.} With the proposed semantic space projection, we project multimodal responses to text semantic space. The distribution entropy in the text semantic space is proficient in indicating LMM uncertainty. Furthermore, uncertainties of each modality are adaptively merged to reveal overall LMM uncertainty.


Through extensive experiments with 18 multimodal benchmarks and 10 LMMs (both open-sourced and closed-source), we validate the effectiveness of Uncertainty-o in accurately capturing the uncertainty of LMMs. The refined uncertainty estimation facilitates various downstream tasks, including hallucination detection, hallucination mitigation, and uncertainty-aware Chain-of-Thought (CoT).
% remark
In summary, our contributions are as follows:
\begin{itemize}
\item \textbf{Unified Framework to Unveil LMM Uncertainty.} We propose Uncertainty-o, which, in a unified manner, reveals one critical property in LMM psychology: LMM uncertainty. Uncertainty-o can seamlessly handle LMMs with various modalities, complex model architectures, and distinct capacity emphases.
\item \textbf{Cookbook for Multimodal Prompt Perturbation.} We propose multimodal prompt perturbation and empirically explore how to perturb the prompt to maximize its contribution to LMM uncertainty estimation.
\item \textbf{Multimodal Uncertainty in Semantic Space.} We propose multimodal semantic uncertainty, explicitly enabling the mining of uncertainty from multimodal generated content via the proposed semantic space mapping.
\end{itemize}

==> sec/2_related.tex <==
\section{Related Work}

\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{method.pdf}
    \caption{
    \textbf{Overview of our Uncertainty-o. \zznote{Given a multimodal prompt and state-of-the-art large multimodal models, \eg, InternVL, OneLLM, and AnyGPT, we perform multimodal prompt perturbation to generate diverse responses. Due to the inherent epistemic uncertainty of these models under perturbation, varied responses are typically obtained. To quantify this uncertainty, we apply semantic clustering on the collected responses and compute their entropy. Specifically, responses are grouped into semantically similar clusters, and the entropy across these clusters is calculated as the final uncertainty measure. Higher entropy indicates greater variability in responses, suggesting lower confidence, while lower entropy reflects higher consistency and thus higher confidence.}}
    }
    \label{fig:method}
\end{figure*}

% My summary
\noindent \textbf{Large Multimodal Model.}
Large Multimodal Models (LMMs)~\cite{caffagni2024revolution} perceive and generate content across a wide range of modalities~\cite{caffagni2024revolution,wu2023multimodal,zhang2024approaching,zhang2024harnessing}, such as text~\cite{achiam2023gpt}, image~\cite{rombach2022high,fei2024vitron}, audio~\cite{zhan2024anygpt}, video~\cite{luo2023videofusion,fei2024video}, and point cloud~\cite{xu2024pointllm}. Fundamental efforts pioneer in building a universal-modal encoder by aligning various modalities to language~\cite{girdhar2023imagebind,lyu2024unibind}. On one hand, various works~\cite{liu2023visual,lin2023video,han2024onellm,xu2024pointllm} focus on enhancing multimodal comprehension ability~\cite{fei2024enhancing}, emphasizing the understanding of complexity~\cite{wu2024visual} and interaction~\cite{zhang2024prompt} between prompts from various modalities. Another line of research focuses on generating multimodal content~\cite{rombach2022high,luo2023videofusion,zhan2024anygpt,lee2024rgb2point}, with an emphasis on the fidelity~\cite{song2024moma,li2024unimo} and diversity~\cite{fang2024puma,tevet2020evaluating} of multimodal responses. Moreover, preliminary attempts~\cite{wu2024next,zhan2024anygpt} try to build an `Any-to-Any' capability~\cite{tang2023any,tang2024codi} in large models, where models can simultaneously comprehend complex multimodal contexts and generate high-fidelity content following those contexts.

% Hallucination of Multimodal Large Language Models: A Survey
\noindent \textbf{LMM Hallucination Detection.}
LMM Hallucination Detection~\cite{bai2024hallucination,huang2024visual} aims for detecting either context-misfollowing~\cite{huang2024survey} or factual mistakes~\cite{akhtar2023multimodal} in generated multimodal reponses. For external-evalutor-based approaches, powerful reponse scorers~\cite{liu2023mitigating,wang2023evaluation} or retrieved real-world fact~\cite{chen2024unified,ding2024retrieve} faciliate hallucination detection. For discrete rule-based checking, CHAIR~\cite{rohrbach2018object} employs the ratio of objects presented in the response relative to a ground truth object list to identify hallucinatory answers, which is limited to fixed object classes. Building on CHAIR, POPE~\cite{li2023evaluating} enhances the prompting technique by focusing on Yes-or-No questions, simplifying process and improving stability. Distinct from existing works, Uncertainty-o harness uncertainty of LMM as an intrinsic indicator of potential hallucination responses.

% https://github.com/Ruiyang-061X/Awesome-MLLM-Uncertainty
\noindent \textbf{Uncertainty in LMM.}
MAP~\cite{ji2022map} proposes a probabilistic distribution encoder to model uncertainty during large model pretraining. VL-Uncertainty~\cite{zhang2024vl} leverages semantic-equivalent perturbations of visual and textual prompts to better capture MLLM uncertainty. DropoutDecoding~\cite{fang2024uncertainty} treats token distribution discrepancies from the average token distribution as uncertainty, dropping tokens with high uncertainty. Calibration-MLLM~\cite{chen2024unveiling} utilizes calibration between different stages of MLLM, such as before and after visual fine-tuning, to reveal uncertainty. IDK~\cite{cohen2025don} introduces an additional special `I Dont Know' token, and quantify uncertainty based on predicted probability of this token. UAL~\cite{wang2024uncertainty} further utilizes uncertainty for large model alignment and improves token convergence in feature space.

==> sec/3_method.tex <==
\section{Method}

\subsection{Multimodal Prompt Perturbation}

\noindent \textbf{Definition 3.1 (Response Semantic Distance).} \textit{The LMM $M$ generate reponses for prompts $x_{i}$ and $x_{j}$ (perturbed from original prompt $x$). For perturbed prompts, the predictions from LMM is $y_{i} = M(x_{i})$, and $y_{j} = M(x_{j})$, respectively. We focus on the LMM's \underline{Epistemic Uncertainty}, which is the uncertainty in the model parameters, $\text{Var}(\theta|x)$. Define the prediction difference $D(x)$ as:}
\begin{equation}
D(x) = \| y_{i} - y_{j} \|,
\end{equation}
\textit{where $\|\cdot\|$ denotes semantic space distance.}

\noindent \textbf{Proposition 3.2 (LMM Uncertainty).} \textit{Response semantic distance $D(x)$ from prompt perturbation is proportional to the square root of the LMM uncertainty:}
\begin{equation}
D(x) \propto \sqrt{\text{Var}(\theta|x)}.
\end{equation}
\textit{Therefore, the prediction semantic distance $D(x)$ can serve as a measure of the LMM uncertainty for a given sample.}

\noindent \textbf{Proof 3.3 (Proportional Theorem).} \textit{Assume LMM parameters $\theta$ are random variables with a prior distribution $P(\theta)$, we get $\theta_{\text{i}}$ and $\theta_{\text{j}}$, which are independently and identically distributed (i.i.d.). Then:}
\begin{equation}
\begin{split}
\mathbb{E}_{\theta|x} \left[ \| \nabla_{\theta} P(y|x, \theta) \cdot (\theta_{\text{i}} - \theta_{j}) \|^2 \right] \approx \\ \mathbb{E}_{\theta|x} \left[ \| \nabla_{\theta} P(y|x, \theta) \|^2 \right] \cdot \mathbb{E}_{\theta|x} \left[ (\theta_{\text{i}} - \theta_{\text{j}})^2 \right].
\end{split}
\end{equation}

\textit{Noting that $\mathbb{E}_{\theta|x} \left[ (\theta_{\text{i}} - \theta_{\text{j}})^2 \right] = 2 \cdot \text{Var}(\theta|x)$:}
\begin{equation}
\begin{split}
\mathbb{E}_{\theta|x} \left[ \| \nabla_{\theta} P(y|x, \theta) \cdot (\theta_{\text{i}} - \theta_{\text{j}}) \|^2 \right] \approx \\ 2 \cdot \mathbb{E}_{\theta|x} \left[ \| \nabla_{\theta} P(y|x, \theta) \|^2 \right] \cdot \text{Var}(\theta|x).
\end{split}
\end{equation}
\textit{Assuming $k = \mathbb{E}_{\theta|x} \left[ \| \nabla_{\theta} P(y|x, \theta) \|^2 \right]$, which is positive:}
\begin{equation}
\mathbb{E}_{\theta|x} \left[ \| \nabla_{\theta} P(y|x, \theta) \cdot (\theta_{\text{i}} - \theta_{\text{j}}) \|^2 \right] \approx 2k \cdot \text{Var}(\theta|x).
\end{equation}
\textit{Assume the difference in predictions can be approximated by a First-order Taylor Expansion:}
\begin{equation}
y_{\text{i}} - y_{\text{j}} \approx \mathbb{E}_{\theta|x} \left[ \nabla_{\theta} P(y|x, \theta) \cdot (\theta_{\text{i}} - \theta_{\text{j}}) \right],
\end{equation}
\textit{where $\nabla_{\theta} P(y|x, \theta)$ is the gradient of $P(y|x, \theta)$ with respect to $\theta$.}
\textit{Thus, prediction semantic distance $D(x)$ from prompt perturbation can be expressed as:}
\begin{equation}
D(x) \approx \sqrt{2k} \cdot \sqrt{\text{Var}(\theta|x)} \propto \sqrt{\text{Var}(\theta|x)}.
\end{equation}

(\textit{Refer to Supplementary Material for detailed proof process.})

Based on our \textit{Proportional Theorem}, we propose semantic-equivalent perturbation for multimodal prompts to cause variances in LMM responses to capture LMM uncertainty. Multimodal prompt perturbation creates semantic-equivalent variations of original multimodal prompts and feeds these variations into the LMM, enabling a sampling process. The variance of sampled answers could effectively illustrate LMM uncertainty.
Specifically, we propose multimodal prompt perturbation across five modalities, including text, image, audio, video, and point cloud. Notably, we also adopt a progressive approach to multimodal prompt perturbation. Each prompt is perturbed gradually, from low to high degrees of perturbation. This strategy introduces different levels of challenge to the LMM. Additionally, perturbations across various input modalities are conducted simultaneously.

In practice, for text prompt, we utilize both LLM-based rephrasing and other rule-based perturbation techniques, \eg, word swapping.
For image prompt, both spatial transformations, such as rotation, and attribute distortions, such as blurring or brightness adjustments, are applied. For audio prompt, we consider perturbing key elements of the audio, such as volume, pitch, and timbre. Temporal features are also considered, with perturbations like temporal shifting applied. For video prompt, both temporal and spatial features are perturbed. For temporal perturbation, techniques like temporal cropping or frame dropping are applied. For spatial features, the process is identical to applying image perturbation to each frame of the video. For point cloud prompt, the 3D characteristics, such as point density and 3D shape, are considered. General techniques like random sampling and point cloud jittering are included.

\vspace{1mm}
\noindent \textbf{Discussion.} \textbf{Why is semantic-equivalent perturbation more effective than inequivalent perturbation?} In semantic-equivalent perturbation, the semantics of all perturbed prompts remain the same. As a result, any fluctuation in answers of LMM directly reflects its uncertainty. On the other hand, semantic-inequivalent perturbation alters the original semantics, and changes in the answers are inevitable, making it difficult to accurately reflect the inherent uncertainty of the LMM. \textbf{Why is prompt perturbation superior to vanilla sampling for capturing LMM uncertainty?} Multimodal prompt perturbation challenges the LMM with prompts that vary at different levels, with larger variations of answers indicating higher uncertainty. In contrast, vanilla sampling typically uses a high temperature during sampling, which tends to induce high uncertainty across all samples. For instance, the LMM could be highly confident in its answer, but the high temperature inevitably causes answer variation, leading to an artificially high uncertainty. 

\begin{table*}[!ht]
    \vspace{-20pt}
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{2.4mm}
    % \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l|ccc|ccc|ccc}
        \toprule
        \multicolumn{10}{c}{\textit{Image Comprehension}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{MMVet~\cite{yu2023mm}} & \multicolumn{3}{c|}{LLaVABench~\cite{liu2023visual}} & \multicolumn{3}{c}{CoCoCap~\cite{chen2015microsoft}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & 52.3 & 55.8 & 13.1 & 54.0 & 78.1 & \underline{11.3} & 51.2 & 71.0 & 23.1 \\ 
        GAVIE~\cite{liu2023mitigating} & 55.4 & 45.2 & 9.4 & 45.3 & 75.2 & 23.8 & 57.7 & \underline{79.6} & 28.9 \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{60.6} & \underline{56.9} & \underline{8.8} & \underline{65.8} & \underline{87.4} & 14.9 & \underline{60.1} & 78.4 & \underline{6.9} \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{63.5} & \textbf{66.4} & \textbf{8.2} & \textbf{68.0} & \textbf{91.3} & \textbf{10.1} & \textbf{65.5} & \textbf{82.5} & \textbf{5.9} \\ 
        \midrule
        \multicolumn{10}{c}{\textit{Video Comprehension}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{MSRVTTQA~\cite{xu2017video}} & \multicolumn{3}{c|}{MSVDQA~\cite{xu2017video}} & \multicolumn{3}{c}{NextQA~\cite{xiao2021next}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & \underline{53.5} & 32.6 & \underline{12.2} & \underline{51.0} & 32.8 & 16.1 & 51.5 & \underline{65.9} & 10.9 \\ 
        GAVIE~\cite{liu2023mitigating} & 50.1 & 33.9 & 18.2 & 39.6 & 30.1 & 20.5 & 47.4 & 60.8 & 11.4 \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & 51.6 & \underline{35.1} & 14.7 & 47.1 & \underline{32.7} & \underline{18.6} & \underline{59.1} & 62.4 & \underline{12.6} \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{55.4} & \textbf{39.2} & \textbf{10.8} & \textbf{52.4} & \textbf{36.3} & \textbf{14.5} & \textbf{67.4} & \textbf{69.0} & \textbf{7.4} \\ 
        \midrule
        \multicolumn{10}{c}{\textit{Audio Comprehension}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{AudioCaps~\cite{kim2019audiocaps}} & \multicolumn{3}{c|}{ClothoV2~\cite{drossos2020clotho}} & \multicolumn{3}{c}{ClothoAQA~\cite{lipping2022clotho}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & 50.9 & 30.2 & 18.6 & 51.2 & 34.1 & 24.2 & 49.2 & 53.5 & 29.0 \\ 
        GAVIE~\cite{liu2023mitigating} & 47.7 & 34.8 & 19.7 & 51.1 & 31.9 & 30.6 & 53.1 & 56.7 & 23.9 \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{50.9} & \underline{42.4} & \underline{16.1} & \underline{62.1} & \underline{38.5} & \underline{23.7} & \underline{56.7} & \underline{60.2} & \underline{17.2} \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{56.7} & \textbf{46.6} & \textbf{12.4} & \textbf{77.7} & \textbf{44.1} & \textbf{21.3} & \textbf{60.4} & \textbf{67.5} & \textbf{11.6} \\ 
        \midrule
        \multicolumn{10}{c}{\textit{Point Cloud Comprehension}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Objaverse~\cite{deitke2023objaverse}} & \multicolumn{3}{c|}{ModelNet~\cite{wu20153d}} & \multicolumn{3}{c}{ShapeNet~\cite{chang2015shapenet}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & 49.5 & 28.0 & 23.1 & 47.1 & \underline{78.0} & 36.1 & 46.4 & 72.1 & 19.7 \\ 
        GAVIE~\cite{liu2023mitigating} & 49.8 & 35.1 & 29.4 & 46.0 & 84.5 & 43.5 & 51.1 & \underline{80.4} & 17.5 \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{50.1} & \underline{38.5} & \underline{26.0} & \underline{52.7} & 79.2 & \underline{39.8} & \underline{54.6} & 73.6 & \underline{20.6} \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{56.9} & \textbf{43.8} & \textbf{18.7} & \textbf{66.5} & \textbf{92.1} & \textbf{31.9} & \textbf{62.3} & \textbf{81.5} & \textbf{13.1} \\ 
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Comprehension Hallucination Detection Results.} Uncertainty-o consistently outperforms strong baselines by a clear margin in LMM hallucination detection. We present comparison results across 12 benchmarks, covering tasks in image, video, audio, and point cloud comprehension. The best results are bolded, and the second-best results are underlined.
    }
    \label{tab:main_comprehension}
\end{table*}


\begin{figure*}[!ht]
    \centering
    \vspace{-10pt}
    \includegraphics[width=\linewidth]{calibration.pdf}
    \caption{
    \textbf{Uncertainty - Error Rate Calibration.} From the comparison between Uncertainty-o and previous methods, we observe that: (1) Compared to Confidence Elicitation, Uncertainty-o effectively avoids the over-confidence problem, which inaccurately assigns low uncertainty (or high confidence) to hallucinatory responses. (2) Compared to Semantic Entropy, Uncertainty-o provides more reliable uncertainty estimation, e.g., the uncertainty is more closely aligned with the error rate in each bin.
    }
    \label{fig:calibration}
    \vspace{-10pt}
\end{figure*}

\subsection{Multimodal Semantic Uncertainty} 

We quantify the variance of these sampled answers to capture the inherent uncertainty of the LMM.
Diverging from mere format-based variance calculations, we opt for variations in answer semantics. To facilitate estimating the variance of sampled answer semantics, the most critical procedure lies in semantic checking between two generated answers. Given this challenge, especially for higher-level modalities, \eg, video, we propose utilizing an off-the-shelf LMM captioner to extract answer semantic and summarize the key points into text captions. Consequently, the challenging multimodal semantic checking is reduced to the more manageable text semantic checking. 

Specifically, for those text captions, we directly prompt the LLM to iteratively check between text answer pairs. For texts with similar semantics, we cluster them into one group. After obtaining the semantic clusters of sampled answers, we consider the discrete distribution of answer semantics and calculate the distribution entropy. Moreover, we normalize the calculated entropy compared to the maximum entropy decided by the sampling time, and obtain estimated LMM uncertainty, with higher values indicating greater LMM uncertainty: 
\begin{equation}
u_{m} = - \sum_{i=1}^{n} p_i \log(p_i) \quad \text{where} \quad p_i = \frac{c_i}{C},
\end{equation}
where $c_i$ is answer count for $i$-th group, $C$ is the total answer count, $u_{m}$ is the estimated uncertainty for certain response modal $m$.
Lastly, uncertainty from each answer modalities is averaged to obtain final LMM uncertainty $u$.

\vspace{1mm}
\noindent \textbf{Discussion.} \textbf{Can multimodal semantic uncertainty extend to more modalities?} Yes. Uncertainty-o proposes a general pipeline for LMM uncertainty estimation. This pipeline is orthogonal to and can benefit from iterations of MLLM. With a more general MLLM, which is capable of parsing the semantic content of additional modalities into textual descriptions, Uncertainty-o can seamlessly estimate uncertainty for those answers in more modalities.  \textbf{Why not directly utilize LMM to check whether two generated multimodal responses are semantically equivalent?} Current MLLMs still lack proficient ability for multimodal semantic checking. We have attempted two methods to utilize MLLM for direct multimodal data semantic checking: (1) Combine two multimodal answers into one and prompt the MLLM to check whether the answers are similar. For example, merge two point clouds into one and conduct shifting so that they do not overlap. However, current MLLMs show unsatisfactory performance. (2) Directly input two answers into MLLM and prompt it to check. We find that many MLLMs still do not support multi-input, such as understanding two audios simultaneously.

\begin{table}[!ht]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{2.4mm}
    % \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        \multicolumn{4}{c}{\textit{Image Generation}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{Flickr~\cite{plummer2015flickr30k}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        GAVIE~\cite{liu2023mitigating} & 52.3 & 67.9 & \underline{12.7} \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{50.8} & \underline{70.1} & 21.5 \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{59.5} & \textbf{74.5} & \textbf{8.3} \\ 
        \midrule
        \multicolumn{4}{c}{\textit{Video Generation}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{MSRVTT~\cite{xu2016msr}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        GAVIE~\cite{liu2023mitigating} & 51.6 & 54.1 & \underline{21.7} \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{54.7} & \underline{60.9} & 23.0 \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{62.1} & \textbf{73.5} & \textbf{15.1} \\ 
        \midrule
        \multicolumn{4}{c}{\textit{Audio Generation}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{VCTK~\cite{Yamagishi2019CSTRVC}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        GAVIE~\cite{liu2023mitigating} & \underline{46.0} & \underline{74.6} & 21.5 \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & 48.1 & 72.8 & \underline{20.6} \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{53.5} & \textbf{81.4} & \textbf{11.3} \\ 
        \midrule
        \multicolumn{4}{c}{\textit{Point Cloud Generation}} \\
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{Pix3D~\cite{sun2018pix3d}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        GAVIE~\cite{liu2023mitigating} & 27.9 & 34.2 & \underline{39.5} \\ 
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{43.6} & \underline{38.8} & 43.5 \\ 
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{51.1} & \textbf{44.2} & \textbf{32.0} \\ 
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Generation Hallucination Detection Results.} Uncertainty-o surpasses previous state-of-the-art methods in detecting hallucinations in various generative tasks, including image generation (Flickr), video generation (MSRVTT), audio generation (VCTK), and point cloud generation (Pix3D).
    }
    \label{tab:main_generation}
\end{table}

\subsection{Uncertainty-Aware Downstream Tasks}

\noindent \textbf{Hallucination Detection.} We treat answers with low uncertainty as non-hallucinatory and those with high uncertainty as hallucinatory. In practice, we first infer LMM using the original prompt to obtain an initial answer. This answer is then compared with the ground truth to determine whether it contains hallucinations. Next, we apply the proposed multimodal prompt perturbation and multimodal semantic uncertainty to estimate uncertainty for its initial answer. Finally, we evaluate the alignment between the estimated uncertainty and actual hallucination using three different metrics: AUROC, AURAC, and ECE.



\begin{table}[!ht]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{2.4mm}
    % \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{\textit{Medical Diagnosis}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & 42.1 & 30.9 & 24.5 \\
        GAVIE~\cite{liu2023mitigating} & 44.2 & 33.6 & 31.5 \\
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{52.4} & \underline{34.5} & \underline{24.1} \\
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{59} & \textbf{40.6} & \textbf{15.3} \\
        \midrule
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{\textit{Embodied Robot}} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & 40.1 & 49.6 & \underline{18.9} \\
        GAVIE~\cite{liu2023mitigating} & 45.2 & 53.6 & 23.5 \\
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{56.2} & \underline{55.9} & 21.1 \\
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{58.2} & \textbf{66.5} & \textbf{12.2} \\
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Hallucination Detection for Safety-Critic Tasks.}
    Uncertainty-o outperforms baselines across all metrics in detecting hallucinations in medical and embodied domains, enhancing safety in real-world applications. (MIMICCXR~\cite{johnson2019mimic})(OpenEQA~\cite{majumdar2024openeqa})
    }
    \label{tab:main_safety}
\end{table}

\begin{table}[!ht]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{2.4mm}
    % \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{l|ccc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{MMVet w. GPT4o} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & 59.5 & \underline{67.8} & 8.7 \\
        GAVIE~\cite{liu2023mitigating} & 59.0 & 65.6 & \underline{8.4} \\
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{62.8} & 64.9 & 9.1 \\
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{67.1} & \textbf{72.6} & \textbf{6.9} \\
        \midrule
        \midrule
        \multirow{2}{*}{Method} & \multicolumn{3}{c}{MSRVTTQA w. QwenVLMax} \\ 
        ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Confidence Elicitation~\cite{xiong2023can} & 54.7 & 39.9 & \underline{11.5} \\
        GAVIE~\cite{liu2023mitigating} & 55.9 & 40.1 & 15.6  \\
        Semantic Entropy~\cite{farquhar2024detecting} & \underline{56.8} & \underline{41.5} & 12.8 \\
        \rowcolor{gray!15} \textbf{Uncertainty-o (ours)} & \textbf{60.1} & \textbf{47.5} & \textbf{8.9} \\
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Hallucination Detection for Closed-Source LMMs.}
    }
    \label{tab:main_close}
\end{table}

\begin{figure*}
    \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{perturbation.pdf}
    \caption{
    \textbf{Empirical Comparison of Different Prompt Perturbations.}
    }
    \label{fig:perturbation}
    \vspace{-10pt}
\end{figure*}


\vspace{1mm}
\noindent \textbf{Hallucination Mitigation.} We formulate hallucination mitigation as an uncertainty-aware, two-stage reasoning process. In the first stage, we prompt the LMM to generate an initial answer, which is then assigned an uncertainty score estimated by Uncertainty-o. After constructing an answer pool with corresponding uncertainties, we select answers with the top-K percent highest uncertainty scores, as these are the most likely to contain hallucinations. In the second stage, we refine these high-uncertainty answers by prompting the LMM with the original prompt, incorporating the uncertainty score into the prompt itself. Specifically, we inform the LMM that its initial answer has a high uncertainty score and instruct it to revise the response due to a potential hallucination. The revised answer is then used as the LMM final output:
\begin{equation}  
y_\text{final} = M(x', y_\text{initial}, u), \quad y_\text{initial} \in \mathbf{Y},
\end{equation}
where \( \mathbf{Y} \) contains selected answers,  \( x' \), \( y_\text{initial} \), and \( u \) refers to updated prompt, initial answer and estimated uncertainty, \( y_\text{final} \) for revised answer. This iterative process helps the LMM refine its responses and improve reliability.



\vspace{1mm}
\noindent \textbf{Uncertainty-Aware Chain-of-Thought.} We leverage Uncertainty-o to enhance the vanilla CoT process. Self-reflection is crucial for LMMs during CoT, and our estimated uncertainty serves as a guiding signal to trigger self-reflection. Specifically, at each reasoning step, in addition to generating an answer, we estimate answer uncertainty. In the subsequent step, we incorporate the previous answer and its uncertainty into the context, explicitly prompting LMM to reflect on its reasoning process when it finds uncertainty is high, as: 
\begin{equation}  
y_t, u_t = M(C_t), \quad C_{t+1} = C_t \cup \{y_t, u_t\} \,,
\end{equation}
where \( y_t \) and \( u_t \) is answer and uncertainty, given the context \( C_t \) at step \( t \). This iterative process helps the LMM refine its responses and improve reliability.





% \begin{table}[!ht]
%     \centering
%     \resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{c|ccc}
%         \toprule
%         \multirow{2}{*}{Perturbation} & \multicolumn{3}{c}{MSRVTTQA} \\ 
%         ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
%         \midrule
%         Spatial Cropping & 50.0 & 33.1 & 14.6 \\ 
%         Video Rotation & 50.4 & 34.9 & 13.2 \\ 
%         Video Flipping & 51.3 & 34.5 & 13.9 \\ 
%         Temporal Cropping & 51.7  & 38.2 & 12.9 \\ 
%         Temporal Shifting & 52.2 & 35.1 & 13.5 \\ 
%         Frame Dropping & 52.4 & 38.0 & 12.1 \\ 
%         Video Blurring & 53.2 & 37.1 & 12.5 \\ 
%         Video Brightness & 54.1 & 36.6 & 11.3 \\ 
%         Adjust Play Speed & \textbf{55.4} & \textbf{39.2} & \textbf{10.8} \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{5pt}
%     \caption{
%     \textbf{Ablation of Video Perturbation.}
%     Perturbation which well-preserves original video semantic, \eg, `Adjust Play Speed' achieves best results.
%     }
%     \label{tab:ablation_video_perturbation}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{c|ccc}
%         \toprule
%         \multirow{2}{*}{Perturbation} & \multicolumn{3}{c}{AudioCaps} \\ 
%         ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
%         \midrule
%         Band Pass Filter & 52.1 & 42.0 & 16.9 \\ 
%         High Pass Filter & 53.0 & 44.3 & 14.5 \\ 
%         Low Pass Filter & 53.4 & 43.1 & 15.4 \\ 
%         Pitch Shift & 54.0 & 45.1 & 14.5 \\ 
%         Time Shift & 54.2 & 45.5 & 15.6 \\ 
%         Add Noise & 54.4 & 46.0 & 12.9 \\ 
%         Time Stretch & 55.1 & 46.4 & 12.6 \\ 
%         Adjust Volume & \textbf{56.7} & \textbf{46.6} & \textbf{12.4} \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{5pt}
%     \caption{
%     \textbf{Ablation of Audio Perturbation.} On average, the benefits of semantic-preserving perturbations are superior than semantic-altering operations.
%     }
%     \label{tab:ablation_audio_perturbation}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \resizebox{0.9\linewidth}{!}{
%     \begin{tabular}{c|ccc}
%         \toprule
%         \multirow{2}{*}{Perturbation} & \multicolumn{3}{c}{Objaverse} \\ 
%         ~ & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
%         \midrule
%         Shearing & 52.5 & 40.3 & 24.9 \\ 
%         Outlier Injection & 53.0 & 40.1 & 23.3 \\ 
%         Jittering & 53.4 & 41.9 & 20.9 \\ 
%         Random Sampling & \textbf{56.9} & \textbf{43.8} & \textbf{18.7} \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{5pt}
%     \caption{
%     \textbf{Ablation of Point Cloud Perturbation.} Similar to the patterns observed in video and audio, perturbations that preserve the original prompt semantics are more effective in eliciting LMM uncertainty.
%     }
%     \label{tab:ablation_point_cloud_perturbation}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{c|ccc}
%         \toprule
%         MLLM Captioner & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
%         \midrule
%         OneLLM & 52.3 & 67.9 & \underline{12.7} \\ 
%         OneLLM & 52.3 & 67.9 & \underline{12.7} \\ 
%         OneLLM & 52.3 & 67.9 & \underline{12.7} \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{5pt}
%     \caption{
%     \textbf{Ablation of MLLM Captioner.}
%     }
%     \label{tab:ablation_mllm_captioner}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \resizebox{0.7\linewidth}{!}{
%     \begin{tabular}{c|ccc}
%         \toprule
%         LLM & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
%         \midrule
%         Qwen & 52.3 & 67.9 & \underline{12.7} \\ 
%         LLaMA & 52.3 & 67.9 & \underline{12.7} \\ 
%         DeepSeek & 52.3 & 67.9 & \underline{12.7} \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{5pt}
%     \caption{
%     \textbf{Ablation of LLM for Text Semantic Clustering.}
%     }
%     \label{tab:ablation_llm}
% \end{table}


% \begin{table}[!ht]
%     \centering
%     \resizebox{0.8\linewidth}{!}{
%     \begin{tabular}{c|ccc}
%         \toprule
%         Text Clustering & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
%         \midrule
%         Semantic & \textbf{55.4} & \textbf{39.2} & \textbf{10.8} \\ 
%         Lexical & 48.0 & 33.2 & \underline{12.7} \\ 
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{5pt}
%     \caption{
%     \textbf{Ablation of Text Clustering.} During semantic uncertainty calculation, clustering based on semantics is more effective than clustering based merely on lexical presentation.
%     }
%     \label{tab:ablation_text_clustering}
% \end{table}



% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|c|c|c|}
%         \toprule
%         \textbf{Video Perturbation} & \textbf{Semantic Equivalent} & \textbf{Acc.} \\ 
%         \midrule
%         Play Speed & ~ & ~ \\ 
%         Temporal Shifting & ~ & ~ \\ 
%         Temporal Cropping & ~ & ~ \\ 
%         Frame Dropping & ~ & ~ \\ 
%         Video Blurring & ~ & ~ \\ 
%         Video Brightness & ~ & ~ \\ 
%         Video Rotation & ~ & ~ \\ 
%         Video Flipping & ~ & ~ \\ 
%         Spatial Cropping & ~ & ~ \\ 
%         \bottomrule
%     \end{tabular}
%     \vspace{5pt}
%     \caption{Ablation - Video Perturbation.}
%     \label{ablation_video_perturbation}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|c|c|c|}
%     \toprule
%     \textbf{Audio Perturbation} & \textbf{Semantic Equivalent} & \textbf{Acc.} \\ 
%     \midrule
%     Time Stretch & ~ & ~ \\ 
%     Time Shift & ~ & ~ \\ 
%     Adjust Volume & ~ & ~ \\ 
%     Pitch Shift & ~ & ~ \\ 
%     Add Noise & ~ & ~ \\ 
%     High Pass Filter & ~ & ~ \\ 
%     Low Pass Filter & ~ & ~ \\ 
%     Band Pass Filter & ~ & ~ \\ 
%     \bottomrule
%     \end{tabular}
%     \vspace{5pt}
%     \caption{Ablation - Audio Perturbation.}
%     \label{ablation_audio_perturbation}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|c|c|c|}
%         \toprule
%         \textbf{Point Cloud Perturbation} & \textbf{Sem. Equiva.} & \textbf{Acc.} \\ 
%         \midrule
%         Rotation & ~ & ~ \\ 
%         Reflecting & ~ & ~ \\ 
%         Scaling & ~ & ~ \\ 
%         Translation & ~ & ~ \\ 
%         Random Sampling & ~ & ~ \\ 
%         Jittering & ~ & ~ \\ 
%         Shearing & ~ & ~ \\ 
%         Outlier Injection & ~ & ~ \\ 
%         \bottomrule
%     \end{tabular}
%     \vspace{5pt}
%     \caption{Ablation - Point Cloud Perturbation.}
%     \label{ablation_point_cloud_perturbation}
% \end{table}


\begin{table}[!t]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{1mm}
    % \resizebox{0.9\linewidth}{!}{
    \begin{tabular}{cccc|ccc}
        \toprule
        Text & Video & Audio & Point & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        \ding{51} & ~ & ~ & ~ & 53.0 & 36.1 & 13.9 \\ 
        ~ & \ding{51} & ~ & ~ & 54.1 & 37.5 & 12.9 \\ 
        \rowcolor{gray!15} \ding{51} & \ding{51} & ~ & ~ & \textbf{55.4} & \textbf{39.2} & \textbf{10.8} \\ 
        \midrule
        \midrule
        \ding{51} & ~ & ~ & ~ & 53.0 & 42.6 & 15.5 \\ 
        ~ & ~ & \ding{51} & ~ & 52.6 & 44.9 & 12.9 \\ 
        \rowcolor{gray!15} \ding{51} & ~ & \ding{51} & ~ & \textbf{56.7} & \textbf{46.6} & \textbf{12.4} \\ 
        \midrule
        \midrule
        \ding{51} & ~ & ~ & ~ & 52.4 & 40.2 & 20.9 \\ 
        ~ & ~ & ~ & \ding{51} & 54.1 & 41.6 & 19.1 \\ 
        \rowcolor{gray!15} \ding{51} & ~ & ~ & \ding{51} &  \textbf{56.9} & \textbf{43.8} & \textbf{18.7}  \\ 
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Ablation of Perturbation Combination.} We observe that combining perturbations for multimodal prompts yield better detection results.
    }
    \label{tab:ablation_combination}
    \vspace{-10pt}
\end{table}

\begin{table}[!t]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{2.4mm}
    % \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|ccc}
        \toprule
        Sampling Time & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        2 & 50.6 & 35.1 & 15.9 \\ 
        3 & 54.2 & 36.9 & 12.4 \\ 
        \rowcolor{gray!15} 5 & \textbf{55.4} & \textbf{39.2} & \textbf{10.8} \\ 
        8 & 52.1 & 38.9 & 11.6 \\ 
        10 & 51.5 & 39.2 & 12.9 \\ 
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Ablation of Sampling Time.} We observe that a moderate sampling time enables the most effective uncertainty estimation.
    }
    \label{tab:ablation_sampling_time}
    \vspace{-10pt}
\end{table}

==> sec/4_exp.tex <==
\section{Experiment}

%\subsection{Setting}

\noindent \textbf{Benchmark.}
We conduct experiments with 14 benchmarks. For the comprehension hallucination task, the benchmarks we adopt are typically QA-type. For images, we utilize MMVet, LLaVABench, and CoCoCap. For video benchmarks, we leverage MSRVTTQA, MSVDQA, and NextQA. For the audio modality, we use ClothV2 and AudioCaps. For point cloud benchmarks, we utilize PointCap and ModelNet. For generation hallucination detection, we use caption-type benchmarks and employ captions as generation prompts. For image generation, we utilize Flickr. For video generation, we utilize MSRVTT. For audio generation, we utilize VCTK. For point cloud generation, we utilize Pix3D, aiming for image-to-point cloud generation.



\begin{table}[!t]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{2.4mm}
    % \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|ccc}
        \toprule
        Pairing Order & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        \rowcolor{gray!15} Progressive & \textbf{55.4} & \textbf{39.2} & \textbf{10.8} \\ 
        Random & 51.1 & 37.2 & 13.9 \\ 
        Shifted & 52.4 & 37.8 & 12.5 \\ 
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Ablation of Pairing Order for Perturbed Multimodal Prompts.} Pairing prompts with similar degrees of perturbation from different modalities in a progressive manner yields the best results.
    }
    \label{tab:ablation_order}
    \vspace{-10pt}
\end{table}


\begin{table}[!t]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{1.5mm}
    % \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{c|ccc}
        \toprule
        Method & AUROC$\uparrow$ & AURAC$\uparrow$ & ECE$\downarrow$ \\ 
        \midrule
        Cycle Consistency & 57.7 & 72.9 & 9.2 \\ 
        \rowcolor{gray!15} Uncertainty-o & \textbf{59.5} & \textbf{74.5} & \textbf{8.3} \\ 
        \bottomrule
    \end{tabular}
    % }
    \vspace{5pt}
    \caption{
    \textbf{Ablation of Cycle Consistency for Generation Hallucination Detection.} Uncertainty-o surpasses cycle consistency, as cycle consistency is constrained by the text similarity scoring capability of the LLM. We experiment on Flickr with Qwen2.5-7B.
    }
    \label{tab:ablation_cycle}
\end{table}


\begin{figure*}
    \centering
    \includegraphics[width=0.9\linewidth]{qualitative.pdf}
    \caption{
    \textbf{Qualitative cases of successful LMM hallucination detection from Uncertainty-o.} Uncertainty-o is proficient at accurately detecting hallucinations when comprehending multimodal prompts, such as vision, audio, and point clouds.
    }
    \label{fig:qualitative}
\end{figure*}

\vspace{1mm}
\noindent \textbf{LMM.}
We experiment with 8 different LMMs capable of understanding and generating various modalities of data. InternVL is a large vision-language model that takes image-text prompts and answers with text. OneLLM is proficient in processing various modal inputs, \eg, audio and point clouds, and outputs text-only responses. PointLLM is specifically designed for real-world point cloud understanding. VideoLLaMA takes videos as prompts and generates text answers. AnyGPT is capable of generating audio and visual data. HunyuanVideo is an industrial-level video generation model, taking text as a prompt. RGB2point realizes point cloud generation by taking a single image. StableDiffusion serves as a text-based image generation model.



\vspace{1mm}
\noindent \textbf{Implementation Details.}
The hallucination detection procedure contains 3 key phases: (1) Initial answer obtaining. The tested LMM is first given the context to generate an initial output. We keep the variation hyper-parameter low at this stage, \eg, low temperature for LLM-based large models and high guidance scale for Diffusion models. The initial answer is compared with the ground truth to decide whether it contains hallucinations. (2) Uncertainty estimation. Initial contexts are perturbed by our proposed multimodal prompt perturbation, according to the modalities they contain. All modal prompts are perturbed simultaneously to various degrees. Different levels of perturbed prompts enable the sampling process. For sampled textual answers, an off-the-shelf LLM, Qwen2.5-7B, clusters them by semantics and calculates entropy as uncertainty. For other modalities' answers, \eg, images, we use OneLLM-7B as a captioner to convert those answers into concise captions. Then, the uncertainty calculation is simplified to vanilla textual semantic uncertainty. (3) Hallucination detection. With hallucination labels from (1) and estimated uncertainties from (2), we utilize AUROC \zznote{xxx}, AURAC\zznote{xxx}, and ECE\zznote{xxx} as hallucination detection metrics. These three metrics comprehensively evaluate the calibration degree between uncertainties and hallucinations.

\subsection{Comparison with State-of-the-Arts}

\noindent \textbf{Comprehension Hallucination Detection.} We compare Uncertainty-o with previous state-of-the-art methods in image, video, audio, and point cloud comprehension hallucination detection tasks (see Tab.~\ref{tab:main_comprehension}). Uncertainty-o yields significant and consistent performance improvements over strong baselines. This validates the general efficacy of the proposed multimodal prompt perturbation in better eliciting and capturing uncertainty, thereby facilitating reliable hallucination detection. Notably, Uncertainty-o surpasses baselines by 9.5\% (AUROC) on MMVet, 8.3\% (AUROC) on NextQA, 14.1\% on ModelNet, and 15.6\% (AUROC) on ClothV2. These significant improvements demonstrate how properly designed prompt perturbation is crucial for refined uncertainty estimation across various modalities.

\noindent \textbf{Generation Hallucination Detection.} We also present comparison results on generation hallucination detection tasks across image, video, audio, and point cloud modalities (see Tab.~\ref{tab:main_generation}). Uncertainty-o consistently shows clear improvements over baseline results. This validates that the interaction between multimodal prompt perturbation and multimodal semantic uncertainty can effectively capture LMM uncertainty and achieve accurate hallucination detection. Specifically, We extend text-only semantic entropy with our multimodal semantic uncertainty, while Uncertainty-o still outperforms this baseline. Moreover, GAVIE is limited by the scoring capability of off-the-shelf evaluators, and Uncertainty-o surpasses it by clear margin.

\noindent \textbf{Safety-Critic Tasks.} We further present a comparison of detection efficacy in the Medical Diagnosis and Embodied Robot domains (see Tab.~\ref{tab:main_safety}). We observe that Uncertainty-o effectively handles the complexity of these real-world applications and outperforms baselines by clear margins. Notably, Uncertainty-o surpasses baselines by 8.8\% in ECE on MIMICCXR and 10.6\% in AURAC on OpenEQA. As a result, the more reliable hallucination detection provided by Uncertainty-o can contribute to safer intelligent system deployments.

\subsection{Ablation Studies and Further Discussions}


\noindent \textbf{Video Perturbation.} We present ablation study of various video perturbations (see Tab.~\ref{tab:ablation_video_perturbation}). We find that perturbations that preserve the original video semantics achieve superior results on average. In contrast, perturbations that alter the original semantics lead to corresponding changes in the answers, resulting in over-estimated uncertainty. As a result, the semantic-preserving perturbations yield the optimal performance.

\noindent \textbf{Audio Perturbation.} We report the ablation of different audio perturbations in Tab.~\ref{tab:ablation_audio_perturbation}. We observe that perturbations that preserve the original audio semantics contribute more to reliable hallucination detection. With the internal semantics intact and the external presentation changed, fluctuations in the sampled answers can directly reflect model uncertainty.

\noindent \textbf{Point Cloud Perturbation.} We show the effectiveness of various point cloud perturbations on hallucination detection performance (see Tab.~\ref{tab:ablation_point_cloud_perturbation}). We observe a similar pattern to that seen in the video and audio domains: operations that preserve the point cloud semantics are more beneficial for accurate hallucination detection.

\noindent \textbf{Perturbation Combination.} We report the ablation of perturbation combinations in Tab.~\ref{tab:ablation_combination}. Concurrently perturbing multimodal prompts yields the best results. This approach effectively mines the uncertainty arising from each modality and contributes to capturing accurate LMM uncertainty.

\noindent \textbf{Sampling Time.} We illustrate the ablation of sampling time during the uncertainty estimation process (see Tab.~\ref{tab:ablation_sampling_time}). With a moderate sampling time, \eg, 5 times, we achieve optimal results. A sampling time that is too small fails to effectively model LMM uncertainty, while excessively high sampling times inevitably lead to over-estimated uncertainty.

\noindent \textbf{Pairing Order.} We present an ablation of pairing order in Tab.~\ref{tab:ablation_order}. For multimodal prompts perturbed to various degrees, pairing them with a similar degree in a progressive manner yields the best results. This approach creates prompt set with challenge level from low to high , effectively eliciting LMM uncertainty.

\noindent \textbf{Text Clustering Manner.} We report the ablation of text clustering methods (see Tab.~\ref{tab:ablation_text_clustering}). Clustering text based on its inherent semantics, rather than merely its lexical presentation, yields the best results.

\noindent \textbf{Uncertainty - Error Rate Calibration.} We further analyze the calibration between estimated uncertainty and actual response error rate (see Fig.~\ref{fig:uncertainty_dis}). Uncertainty-o achieves the most calibrated uncertainty distribution with the answer error rate. In contrast, Confidence Elicitation suffers from the over-confidence problem, as its uncertainty is directly regressed by the LMM itself. Semantic Entropy achieves suboptimal calibration due to the lack of perturbation on multimodal prompts.

\noindent \textbf{Successful Comprehension Hallucination Detection.} We present successful comprehension detection cases in Fig.~\ref{fig:qualitative_perturbation}. With the proposed multimodal prompt perturbation, Uncertainty-o achieves reliable uncertainty estimation, ultimately leading to accurate hallucination detection.

\noindent \textbf{Successful Generation Hallucination Detection.} We also present case studies for generation hallucination detection in Fig.~\ref{fig:generation_case}. Our proposed multimodal semantic uncertainty effectively mines uncertainty from multimodal responses and contributes to the identification of generation hallucination.


==> sec/5_conclusion.tex <==
\section{Conclusion}

Recently, with the widespread and rapid deployment of Large Multimodal Models (LMMs) in real-world applications, concerns about the safety of these models have emerged. Among the various indicators of LMM reliability, we argue that their intrinsic uncertainty remains under-explored. In this paper, we attempt to answer three critical questions: (1) How can we systematically unveil the uncertainty of LMMs capable of perceiving and generating multimodal content? (2) How can we handle the increasing complexity in multimodal prompts, which lead to heightened LMM uncertainty? (3) How can we extract uncertainty from multimodal responses, beyond just text answers? To address these questions, (1) we propose Uncertainty-o, a unified and extensible framework to unveil uncertainty in LMMs, capable of perceiving and generating 5 modalities: text, image, video, audio, and point cloud. (2) We introduce multimodal prompt perturbation and empirically demonstrate that perturbation in a semantically-preserving manner is more effective for capturing LMM uncertainty. (3) We introduce multimodal semantic uncertainty, effectively mining uncertainty from multimodal generated responses. Extensive experiments and analysis validate the superiority of Uncertainty-o in accurately estimating LMM uncertainty and enabling reliable hallucination detection.
